Error Bounds for Flow Matching Methods

Score-based generative models are a popular class of generative modelling techniques relying on stochastic differential equations (SDE). From their inception, it was realized that it was also possible to perform generation using ordinary differential equations (ODE) rather than SDE. This led to the introduction of the probability flow ODE approach and denoising diffusion implicit models. Flow matching methods have recently further extended these ODE-based approaches and approximate a flow between two arbitrary probability distributions. Previous work derived bounds on the approximation error of diffusion models under the stochastic sampling regime, given assumptions on the $L^2$ loss. We present error bounds for the flow matching procedure using fully deterministic sampling, assuming an $L^2$ bound on the approximation error and a certain regularity condition on the data distributions.

==> old.tex <==


@techreport{pulido2011semimartingales,
author = {Pulido, Sergio},
institution = {Carnegie Mellon University},
title = {{Semimartingales and stochastic integration}},
url = {https://www.andrew.cmu.edu/user/calmost/pdfs/21-882-int{\_}lec.pdf},
year = {2011}
}
@techreport{dong2003feller,
author = {Dong, Rui},
institution = {UC Berkeley},
title = {{Feller Processes and Semigroups}},
url = {https://www.stat.berkeley.edu/{~}pitman/s205s03/lecture27.pdf},
year = {2003}
}
@techreport{vanhandel2014probability,
author = {{Van Handel}, Ramon},
institution = {Princeton University},
title = {{Probability in High Dimension}},
year = {2016}
}
@article{radford2019language,
author = {Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
title = {{Language Models are Unsupervised Multitask Learners}},
year = {2019}
}
@book{yosida1965functional,
author = {Yosida, K{\"{o}}saku},
publisher = {Springer Science {\&} Business Media},
title = {{Functional Analyis}},
year = {1965}
}
@book{karatzas1991brownian,
author = {Karatzas, Ioannis and Shreve, Steven E.},
publisher = {Springer Science {\&} Business Media},
title = {{Brownian Motion and Stochastic Calculus}},
year = {1991}
}
@book{schilling2012brownian,
author = {Schilling, Ren{\'{e}} L and Partzsch, Lothar},
publisher = {De Gruyter},
title = {{Brownian Motion: An Introduction to Stochastic Processes}},
year = {2012}
}
@book{taylor2011partial,
author = {Taylor, Michael E},
isbn = {9781441970558},
publisher = {Springer},
title = {{Partial Differential Equations I: Basic Theory}},
year = {2011}
}
@inproceedings{goodfellow2014generative,
archivePrefix = {arXiv},
arxivId = {1406.2661v1},
author = {Goodfellow, Ian J and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1406.2661v1},
title = {{Generative Adversarial Nets}},
year = {2014}
}
@inproceedings{tashiro2021csdi,
archivePrefix = {arXiv},
arxivId = {2107.03502},
author = {Tashiro, Yusuke and Song, Jiaming and Song, Yang and Ermon, Stefano},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.2107.03502},
eprint = {2107.03502},
publisher = {Neural information processing systems foundation},
title = {{CSDI: Conditional Score-based Diffusion Models for Probabilistic Time Series Imputation}},
volume = {30},
year = {2021}
}
@inproceedings{bengio2013generalized,
archivePrefix = {arXiv},
arxivId = {1305.6663},
author = {Bengio, Yoshua and Yao, Li and Alain, Guillaume and Vincent, Pascal},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.1305.6663},
eprint = {1305.6663},
month = {may},
publisher = {Neural information processing systems foundation},
title = {{Generalized Denoising Auto-Encoders as Generative Models}},
year = {2013}
}
@inproceedings{campbell2022continuous,
archivePrefix = {arXiv},
arxivId = {2205.14987},
author = {Campbell, Andrew and Benton, Joe and {De Bortoli}, Valentin and Rainforth, Tom and Deligiannidis, George and Doucet, Arnaud},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.2205.14987},
eprint = {2205.14987},
title = {{A Continuous Time Framework for Discrete Denoising Models}},
year = {2022}
}
@inproceedings{song2020improved,
archivePrefix = {arXiv},
arxivId = {2006.09011},
author = {Song, Yang and Ermon, Stefano},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.2006.09011},
eprint = {2006.09011},
publisher = {Neural information processing systems foundation},
title = {{Improved Techniques for Training Score-Based Generative Models}},
volume = {2020-Decem},
year = {2020}
}
@inproceedings{song2019generative,
archivePrefix = {arXiv},
arxivId = {1907.05600},
author = {Song, Yang and Ermon, Stefano},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.1907.05600},
eprint = {1907.05600},
publisher = {Neural information processing systems foundation},
title = {{Generative Modeling by Estimating Gradients of the Data Distribution}},
volume = {32},
year = {2019}
}
@inproceedings{debortoli2021diffusion,
archivePrefix = {arXiv},
arxivId = {2106.01357},
author = {{De Bortoli}, Valentin and Thornton, James and Heng, Jeremy and Doucet, Arnaud},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2106.01357},
title = {{Diffusion Schr{\"{o}}dinger Bridge with Applications to Score-Based Generative Modeling}},
year = {2021}
}
@inproceedings{debortoli2022riemannian,
archivePrefix = {arXiv},
arxivId = {2202.02763},
author = {{De Bortoli}, Valentin and Mathieu, Emile and Hutchinson, Michael and Thornton, James and Teh, Yee Whye and Doucet, Arnaud},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.2202.02763},
eprint = {2202.02763},
title = {{Riemannian Score-Based Generative Modeling}},
year = {2022}
}
@inproceedings{huang2022riemannian,
archivePrefix = {arXiv},
arxivId = {2208.07949v1},
author = {Huang, Chin-Wei and Aghajohari, Milad and Bose, Avishek Joey and Panangaden, Prakash and Courville, Aaron},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2208.07949v1},
title = {{Riemannian Diffusion Models}},
year = {2022}
}
@inproceedings{kingma2021variational,
archivePrefix = {arXiv},
arxivId = {2107.00630v3},
author = {Kingma, Diederik P and Salimans, Tim and Poole, Ben and Ho, Jonathan},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2107.00630v3},
title = {{Variational Diffusion Models}},
year = {2021}
}
@inproceedings{hoogeboom2019integer,
author = {Hoogeboom, Emiel and Peters, Jorn W T and {Van Den Berg}, Rianne and Welling, Max},
booktitle = {Advances in Neural Information Processing Systems},
title = {{Integer Discrete Flows and Lossless Compression}},
year = {2019}
}
@inproceedings{vaswani2017attention,
archivePrefix = {arXiv},
arxivId = {1706.03762v5},
author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1706.03762v5},
title = {{Attention Is All You Need}},
year = {2017}
}
@inproceedings{brown2020language,
archivePrefix = {arXiv},
arxivId = {2005.14165},
author = {Brown, Tom B and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel M and Wu, Jeffrey and Winter, Clemens and Hesse, Christopher and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arxiv.2005.14165},
eprint = {2005.14165},
title = {{Language Models are Few-Shot Learners}},
year = {2020}
}
@inproceedings{dhariwal2021diffusion,
archivePrefix = {arXiv},
arxivId = {2105.05233},
author = {Dhariwal, Prafulla and Nichol, Alex},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2105.05233},
title = {{Diffusion Models Beat GANs on Image Synthesis}},
year = {2021}
}
@inproceedings{austin2021structured,
archivePrefix = {arXiv},
arxivId = {2107.03006},
author = {Austin, Jacob and Johnson, Daniel D and Ho, Jonathan and Tarlow, Daniel and {Van Den Berg}, Rianne},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2107.03006},
title = {{Structured Denoising Diffusion Models in Discrete State-Spaces}},
year = {2021}
}
@inproceedings{ho2020denoising,
archivePrefix = {arXiv},
arxivId = {2006.11239},
author = {Ho, Jonathan and Jain, Ajay and Abbeel, Pieter},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2006.11239},
title = {{Denoising Diffusion Probabilistic Models}},
year = {2020}
}
@inproceedings{hoogeboom2021argmax,
archivePrefix = {arXiv},
arxivId = {2102.05379},
author = {Hoogeboom, Emiel and Nielsen, Didrik and Jaini, Priyank and Forr{\'{e}}, Patrick and Welling, Max},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2102.05379},
title = {{Argmax Flows and Multinomial Diffusion: Learning Categorical Distributions}},
year = {2021}
}
@inproceedings{huang2021variational,
archivePrefix = {arXiv},
arxivId = {2106.02808},
author = {Huang, Chin-Wei and Lim, Jae Hyun and Courville, Aaron},
booktitle = {Advances in Neural Information Processing Systems},
doi = {10.48550/arXiv.2106.02808},
eprint = {2106.02808},
title = {{A Variational Perspective on Diffusion-Based Generative Models and Score Matching}},
year = {2021}
}
@inproceedings{song2021maximum,
archivePrefix = {arXiv},
arxivId = {2101.09258},
author = {Song, Yang and Durkan, Conor and Murray, Iain and Ermon, Stefano},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2101.09258},
title = {{Maximum Likelihood Training of Score-Based Diffusion Models}},
year = {2021}
}
@article{oord2016wavenet,
archivePrefix = {arXiv},
arxivId = {1609.03499},
author = {van den Oord, Aaron and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
doi = {10.48550/arxiv.1609.03499},
eprint = {1609.03499},
journal = {arXiv preprint arXiv:1609.03499},
title = {{WaveNet: A Generative Model for Raw Audio}},
year = {2016}
}
@article{cattiaux2021time,
archivePrefix = {arXiv},
arxivId = {2104.07708v1},
author = {Cattiaux, Patrick and Conforti, Giovanni and Gentil, Ivan and L{\'{e}}onard, Christian},
eprint = {2104.07708v1},
journal = {arXiv preprint arXiv:2104.07708},
title = {{Time reversal of diffusion processes under a finite entropy condition}},
year = {2021}
}
@article{nachmani2021zero,
archivePrefix = {arXiv},
arxivId = {2111.01471},
author = {Nachmani, Eliya and Dovrat, Shaked},
doi = {10.48550/arxiv.2111.01471},
eprint = {2111.01471},
journal = {arXiv preprint arXiv:2111.01471},
title = {{Zero-Shot Translation using Diffusion Models}},
year = {2021}
}
@article{batzolis2021conditional,
archivePrefix = {arXiv},
arxivId = {2111.13606},
author = {Batzolis, Georgios and Stanczuk, Jan and Sch{\"{o}}nlieb, Carola-Bibiane and Etmann, Christian},
doi = {10.48550/arxiv.2111.13606},
eprint = {2111.13606},
journal = {arXiv preprint arXiv:2111.13606},
title = {{Conditional Image Generation with Score-Based Diffusion Models}},
year = {2021}
}
@article{ramesh2022hierarchical,
archivePrefix = {arXiv},
arxivId = {2204.06125},
author = {Ramesh, Aditya and Dhariwal, Prafulla and Nichol, Alex and Chu, Casey and Chen, Mark},
doi = {10.48550/arxiv.2204.06125},
eprint = {2204.06125},
journal = {arXiv preprint arXiv:2204.06125},
title = {{Hierarchical Text-Conditional Image Generation with CLIP Latents}},
year = {2022}
}
@article{saharia2022photorealistic,
archivePrefix = {arXiv},
arxivId = {2205.11487},
author = {Saharia, Chitwan and Chan, William and Saxena, Saurabh and Li, Lala and Whang, Jay and Denton, Emily and Ghasemipour, Seyed Kamyar Seyed and Ayan, Burcu Karagol and Mahdavi, S Sara and Lopes, Rapha Gontijo and Salimans, Tim and Ho, Jonathan and Fleet, David J and Norouzi, Mohammad},
doi = {10.48550/arxiv.2205.11487},
eprint = {2205.11487},
journal = {arXiv preprint arXiv:2205.11487},
title = {{Photorealistic Text-to-Image Diffusion Models with Deep Language Understanding}},
year = {2022}
}
@inproceedings{liu2022flow,
archivePrefix = {arXiv},
arxivId = {2209.03003v1},
author = {Liu, Xingchao and Gong, Chengyue and Liu, Qiang},
eprint = {2209.03003v1},
booktitle = {International Conference on Learning Representations},
title = {{Flow Straight and Fast: Learning to Generate and Transfer Data with Rectified Flow}},
year = {2023}
}

@inproceedings{chen2022sampling,
archivePrefix = {arXiv},
author = {Chen, Sitan and Chewi, Sinho and Li, Jerry and Li, Yuanzhi and Salim, Adil and Zhang, Anru R},
eprint = {2209.11215},
booktitle = {International Conference on Learning Representations},
title = {{Sampling is as easy as learning the score: theory for diffusion models with minimal data assumptions}},
year = {2023}
}
@inproceedings{lipman2022flow,
archivePrefix = {arXiv},
arxivId = {2210.02747v2},
author = {Lipman, Yaron and Chen, Ricky T Q and Ben-Hamu, Heli and Nickel, Maximilian and Le, Matt and Ai, Meta},
eprint = {2210.02747v2},
booktitle = {International Conference on Learning Representations},
title = {{Flow matching for generative modeling}},
year = {2023}
}

@article{palmowski2002technique,
author = {Palmowski, Zbigniew and Rolski, Tomasz},
journal = {Bernoulli},
number = {6},
pages = {767--785},
title = {{A Technique for Exponential Change of Measure for Markov Processes}},
volume = {8},
year = {2002}
}
@article{hyvarinen2007some,
author = {Hyv{\"{a}}rinen, Aapo},
doi = {10.1016/j.csda.2006.09.003},
journal = {Computational Statistics and Data Analysis},
pages = {2499 -- 2512},
title = {{Some extensions of score matching}},
volume = {51},
year = {2007}
}
@inproceedings{leach2022denoising,
author = {Leach, Adam and Schmon, Sebastian M and Degiacomi, Matteo T and Willcocks, Chris G},
booktitle = {ICLR 2022 Workshop on Geometrical and Topological Representation Learning},
title = {{Denoising Diffusion Probabilistic Models on SO(3) for Rotational Alignment}},
year = {2022}
}
@article{saharia2022image,
archivePrefix = {arXiv},
arxivId = {2104.07636},
author = {Saharia, Chitwan and Ho, Jonathan and Chan, William and Salimans, Tim and Fleet, David J and Norouzi, Mohammad},
doi = {10.1109/TPAMI.2022.3204461},
eprint = {2104.07636},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
pages = {1--14},
title = {{Image Super-Resolution via Iterative Refinement}},
year = {2022}
}
@inproceedings{karras2020analyzing,
archivePrefix = {arXiv},
arxivId = {1912.04958},
author = {Karras, Tero and Laine, Samuli and Aittala, Miika and Hellsten, Janne and Lehtinen, Jaakko and Aila, Timo},
booktitle = {IEEE/CVF Conference on Computer Vision and Pattern Recognition},
doi = {10.48550/arxiv.1912.04958},
eprint = {1912.04958},
pages = {8110--8119},
title = {{Analyzing and Improving the Image Quality of StyleGAN}},
year = {2020}
}
@inproceedings{vignac2023digress,
archivePrefix = {arXiv},
arxivId = {2209.14734},
author = {Vignac, Clement and Krawczuk, Igor and Siraudin, Antoine and Wang, Bohan and Cevher, Volkan and Frossard, Pascal},
booktitle = {International Conference on Learning Representations},
eprint = {2209.14734},
title = {{DiGress: Discrete Denoising diffusion for graph generation}},
year = {2023}
}
@inproceedings{albergo2023building,
author = {Albergo, Michael S and Vanden-Eijnden, Eric},
booktitle = {International Conference on Learning Representations},
title = {{Building Normalizing Flows with Stochastic Interpolants}},
year = {2023}
}
@inproceedings{sun2023score,
author = {Sun, Haoran and Yu, Lijun and Dai, Bo and Schuurmans, Dale and Dai, Hanjun},
booktitle = {International Conference on Learning Representations},
title = {{Score-based Continuous-time Discrete Diffusion Models}},
year = {2023}
}
@inproceedings{trippe2023diffusion,
archivePrefix = {arXiv},
arxivId = {2206.04119},
author = {Trippe, Brian L and Yim, Jason and Tischer, Doug and Baker, David and Broderick, Tamara and Barzilay, Regina and Jaakkola, Tommi},
booktitle = {International Conference on Learning Representations},
doi = {10.48550/arxiv.2206.04119},
eprint = {2206.04119},
title = {{Diffusion probabilistic modeling of protein backbones in 3D for the motif-scaffolding problem}},
year = {2023}
}
@inproceedings{savinov2022step,
archivePrefix = {arXiv},
arxivId = {2112.06749},
author = {Savinov, Nikolay and Chung, Junyoung and Binkowski, Mikolaj and Elsen, Erich and van den Oord, Aaron},
booktitle = {International Conference on Learning Representations},
eprint = {2112.06749},
title = {{Step-unrolled Denoising Autoencoders for Text Generation}},
year = {2022}
}
@inproceedings{song2021denoising,
archivePrefix = {arXiv},
arxivId = {2010.02502},
author = {Song, Jiaming and Meng, Chenlin and Ermon, Stefano},
booktitle = {International Conference on Learning Representations},
eprint = {2010.02502},
title = {{Denoising Diffusion Implicit Models}},
year = {2021}
}
@inproceedings{kingma2014autoencoding,
archivePrefix = {arXiv},
arxivId = {1312.6114v10},
author = {Kingma, Diederik P and Welling, Max},
booktitle = {International Conference on Learning Representations},
doi = {10.48550/arXiv.1312.6114},
eprint = {1312.6114v10},
title = {{Auto-Encoding Variational Bayes}},
year = {2014}
}
@inproceedings{song2021score,
archivePrefix = {arXiv},
arxivId = {2011.13456},
author = {Song, Yang and Sohl-Dickstein, Jascha and Kingma, Diederik P and Kumar, Abhishek and Ermon, Stefano and Poole, Ben},
booktitle = {International Conference on Learning Representations},
eprint = {2011.13456},
title = {{Score-Based Generative Modeling through Stochastic Differential Equations}},
year = {2021}
}
@inproceedings{rezende2015variational,
archivePrefix = {arXiv},
arxivId = {1505.05770},
author = {Rezende, Danilo Jimenez and Mohamed, Shakir},
booktitle = {International Conference on Machine Learning},
eprint = {1505.05770},
title = {{Variational Inference with Normalizing Flows}},
year = {2015}
}
@inproceedings{hoogeboom2022equivariant,
archivePrefix = {arXiv},
arxivId = {2203.17003v1},
author = {Hoogeboom, Emiel and Satorras, Victor Garcia and Vignac, Cl{\'{e}}ment and Welling, Max},
booktitle = {International Conference on Machine Learning},
eprint = {2203.17003v1},
title = {{Equivariant Diffusion for Molecule Generation in 3D}},
year = {2022}
}
@inproceedings{sohldickstein2015deep,
author = {Sohl-Dickstein, Jascha and Weiss, Eric A and Maheswaranathan, Niru and Ganguli, Surya},
booktitle = {International Conference on Machine Learning},
title = {{Deep Unsupervised Learning Using Nonequilibrium Thermodynamics}},
year = {2015}
}
@article{hyvarinen2005estimation,
author = {Hyv{\"{a}}rinen, Aapo},
journal = {Journal of Machine Learning Research},
number = {24},
pages = {695--709},
title = {{Estimation of Non-Normalized Statistical Models by Score Matching}},
volume = {6},
year = {2005}
}
@article{alain2014what,
author = {Alain, Guillaume and Bengio, Yoshua},
journal = {Journal of Machine Learning Research},
number = {110},
pages = {3743--3773},
title = {{What Regularized Auto-Encoders Learn from the Data-Generating Distribution}},
volume = {15},
year = {2014}
}
@book{levin2009markovchains,
author = {Levin, David and Peres, Yuval and Wilmer, Elizabeth},
booktitle = {Markov Chains and Mixing Times},
doi = {10.1090/mbk/058},
isbn = {978-0-8218-4739-8},
publisher = {American Mathematical Society},
title = {{Markov Chains and Mixing Times}},
year = {2009}
}
@article{vincent2011connection,
author = {Vincent, Pascal},
journal = {Neural Computation},
number = {7},
pages = {1661--1674},
title = {{A Connection Between Score Matching and Denoising Autoencoders}},
volume = {23},
year = {2011}
}
@book{metivier1982semimartingales,
author = {M{\'{e}}tivier, Michel},
booktitle = {Semimartingales},
doi = {10.1515/9783110845563},
isbn = {9783110845563},
publisher = {De Gruyter},
title = {{Semimartingales}},
year = {1982}
}
@article{ethier1993fleming,
author = {Ethier, S N and Kurtz, Thomas G},
doi = {10.1137/0331019},
journal = {SIAM Journal on Control and Optimization},
number = {2},
pages = {345--386},
title = {{Fleming-Viot processes in population genetics}},
volume = {31},
year = {1993}
}
@article{conforti2022time,
archivePrefix = {arXiv},
arxivId = {2104.10948v2},
author = {Conforti, Giovanni and L{\'{e}}onard, Christian},
doi = {10.1016/j.spa.2021.10.002},
eprint = {2104.10948v2},
journal = {Stochastic Processes and their Applications},
pages = {85--124},
title = {{Time reversal of Markov processes with jumps under a finite entropy condition}},
volume = {144},
year = {2022}
}
@article{anderson1982reverse,
author = {Anderson, Brian D O},
doi = {10.1016/0304-4149(82)90051-5},
journal = {Stochastic Processes and their Applications},
number = {3},
pages = {313--326},
title = {{Reverse-time diffusion equation models}},
volume = {12},
year = {1982}
}
@article{ethier1993transition,
author = {Ethier, S N and Griffiths, R C},
doi = {10.1214/aop/1176989131},
journal = {The Annals of Probability},
number = {3},
pages = {1571--1590},
title = {{The Transition Function of a Fleming-Viot Process}},
volume = {21},
year = {1993}
}
@article{molchanov1968strong,
author = {Molchanov, S A},
doi = {10.1137/1113056},
journal = {Theory of Probability {\&} Its Applications},
number = {3},
pages = {471--475},
title = {{Strong Feller Property of Diffusion Processes on Smooth Manifolds}},
volume = {13},
year = {1968}
}
@inproceedings{shi2022conditional,
archivePrefix = {arXiv},
arxivId = {2202.13460},
author = {Shi, Yuyang and {De Bortoli}, Valentin and Deligiannidis, George and Doucet, Arnaud},
booktitle = {Uncertainty in Artificial Intelligence},
doi = {10.48550/arxiv.2202.13460},
eprint = {2202.13460},
title = {{Conditional Simulation Using Diffusion Schr{\"{o}}dinger Bridges}},
year = {2022}
}
@inproceedings{lyu2009interpretation,
author = {Lyu, Siwei},
booktitle = {Uncertainty in Artificial Intelligence},
title = {{Interpretation and generalization of score matching}},
year = {2009}
}
@inproceedings{song2019sliced,
author = {Song, Yang and Garg, Sahaj and Shi, Jiaxin and Ermon, Stefano},
booktitle = {Uncertainty in Artificial Intelligence},
doi = {10.48550/arXiv.1905.07088},
title = {{Sliced Score Matching: A Scalable Approach to Density and Score Estimation}},
year = {2019}
}
@misc{jagvaral2022diffusion,
author = {Jagvaral, Yesukhei and Lanusse, Francois and Mandelbaum, Rachel},
booktitle = {under review},
title = {{Diffusion Generative Models on SO(3)}},
year = {2022}
}
@inproceedings{grathwohl2019ffjord,
archivePrefix = {arXiv},
arxivId = {1810.01367v3},
author = {Grathwohl, Will and Chen, Ricky T Q and Bettencourt, Jesse and Sutskever, Ilya and Duvenaud, David},
booktitle = {International Conference on Learning Representations},
eprint = {1810.01367v3},
title = {{FFJORD: Free-form Continuous Dynamics for Scalable Reverse Generative Models}},
year = {2019}
}
@inproceedings{chen2018neural,
archivePrefix = {arXiv},
arxivId = {1806.07366},
author = {Chen, Ricky T Q and Rubanova, Yulia and Bettencourt, Jesse and Duvenaud, David},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {1806.07366},
title = {{Neural Ordinary Differential Equations}},
year = {2018}
}
@inproceedings{rozen2021moser,
archivePrefix = {arXiv},
arxivId = {2108.08052},
author = {Rozen, Noam and Grover, Aditya and Nickel, Maximilian and Lipman, Yaron},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2108.08052},
title = {{Moser Flow: Divergence-based Generative Modeling on Manifolds}},
year = {2021}
}
@article{debortoli2022convergence,
archivePrefix = {arXiv},
arxivId = {2208.05314},
author = {{De Bortoli}, Valentin},
eprint = {2208.05314},
journal = {Transactions on Machine Learning Research},
title = {{Convergence of denoising diffusion models under the manifold hypothesis}},
year = {2023}
}
@inproceedings{benhamu2022matching,
archivePrefix = {arXiv},
arxivId = {2207.04711},
author = {Ben-Hamu, Heli and Cohen, Samuel and Bose, Joey and Amos, Brandon and Grover, Aditya and Nickel, Maximilian and Chen, Ricky T Q and Lipman, Yaron},
booktitle = {International Conference on Machine Learning},
eprint = {2207.04711},
title = {{Matching Normalizing Flows and Probability Paths on Manifolds}},
year = {2022}
}
@article{shi2023diffusion,
archivePrefix = {arXiv},
arxivId = {2303.16852v1},
author = {Shi, Yuyang and {De Bortoli}, Valentin and Campbell, Andrew and Doucet, Arnaud},
eprint = {2303.16852v1},
journal = {arXiv preprint arXiv:2303.16852},
title = {{Diffusion Schr{\"{o}}dinger Bridge Matching}},
year = {2023}
}
@inproceedings{chen2023restoration,
author = {Chen, Sitan and Daras, Giannis and Dimakis, Alexandros G},
booktitle = {International Conference on Machine Learning},
title = {{Restoration-Degradation Beyond Linear Diffusions: A Non-Asymptotic Analysis For DDIM-Type Samplers}},
year = {2023}
}
@article{albergo2023stochastic,
archivePrefix = {arXiv},
arxivId = {2303.08797},
author = {Albergo, Michael S and Boffi, Nicholas M and Vanden-Eijnden, Eric},
eprint = {2303.08797},
journal = {arXiv preprint arXiv:2303.08797},
title = {{Stochastic Interpolants: A Unifying Framework for Flows and Diffusions}},
year = {2023}
}
@article{peluchetti2021non,
author = {Peluchetti, Stefano},
title = {{Non-Denoising Forward-Time Diffusions}},
year = {2021}
}
@inproceedings{karras2022elucidating,
archivePrefix = {arXiv},
arxivId = {2206.00364},
author = {Karras, Tero and Aittala, Miika and Aila, Timo and Laine, Samuli},
booktitle = {Advances in Neural Information Processing Systems},
eprint = {2206.00364},
title = {{Elucidating the Design Space of Diffusion-Based Generative Models}},
year = {2022}
}
@inproceedings{salimans2022progressive,
archivePrefix = {arXiv},
arxivId = {2202.00512},
author = {Salimans, Tim and Ho, Jonathan},
booktitle = {International Conference on Learning Representations},
eprint = {2202.00512},
title = {{Progressive Distillation for Fast Sampling of Diffusion Models}},
year = {2022}
}
@book{groebner1960die,
author = {Gr{\"{o}}bner, Wolfgang},
publisher = {Berlin: VEB Deutscher Verlag der Wissenschaften},
title = {{Die Lie-Reihen und ihre Anwendungen}},
year = {1960}
}
@article{alekseev1961estimate,
author = {Alekseev, Vladimir M},
journal = {Vestn. Mosk. Univ. Ser. I. Math. Mekh},
pages = {28--36},
title = {{An estimate for the perturbations of the solutions of ordinary differential equations}},
volume = {2},
year = {1961}
}
@article{brascamp1976extensions,
author = {Brascamp, Herm Jan and Lieb, Elliott H},
journal = {Journal of Functional Analysis},
number = {4},
pages = {366--389},
title = {{On extensions of the Brunn--Minkowski and Pr{\'{e}}kopa--Leindler theorems, including inequalities for log concave functions, and with an application to the diffusion equation}},
volume = {22},
year = {1976}
}
@inproceedings{popov2021grad,
author = {Vadim Popov and Ivan Vovk and Vladimir Gogoryan and Tasnima Sadekova and Mikhail Kudinov},
booktitle = {International Conference on Machine Learning},
title = {{Grad-TTS: A Diffusion Probabilistic Model for Text-to-Speech}},
year = {2021},
}
@inproceedings{lee2022convergence,
author = {Lee, Holden and Lu, Jianfeng and Tan, Yixin},
booktitle = {Advances in Neural Information Processing Systems},
title = {{Convergence for score-based generative modeling with polynomial complexity}},
year = {2022}
}
@inproceedings{lee2023convergence,
author = {Holden Lee and Jianfeng Lu and Yixin Tan},
booktitle = {International Conference on Algorithmic Learning Theory},
pages = {946-985},
title = {Convergence of score-based generative modeling for general data distributions},
year = {2023},
}
@inproceedings{zhang2022fast,
author = {Qinsheng Zhang and Yongxin Chen},
booktitle = {International Conference on Learning Representations},
title = {Fast Sampling of Diffusion Models with Exponential Integrator},
year = {2023},
}
@article{alaoui2022information,
archivePrefix = {arXiv},
arxivId = {2109.00709},
author = {Alaoui, Ahmed El and Montanari, Andrea},
eprint = {2109.00709},
journal = {IEEE Transactions on Information Theory},
number = {11},
pages = {7423--7426},
title = {{An Information-Theoretic View of Stochastic Localization}},
volume = {68},
year = {2022}
}
@article{eldan2020taming,
archivePrefix = {arXiv},
arxivId = {1811.11530},
author = {Eldan, Ronen},
eprint = {1811.11530},
journal = {Probability Theory and Related Fields},
number = {3-4},
pages = {737--755},
title = {{Taming correlations through entropy-efficient measure decompositions with applications to mean-field approximation}},
volume = {176},
year = {2020}
}
@article{chen2023probability,
author = {Sitan Chen and Sinho Chewi and Holden Lee and Yuanzhi Li and Jianfeng Lu and Adil Salim},
journal = {arXiv preprint arXiv:2305.11798},
title = {{The probability flow ODE is provably fast}},
year = {2023},
}

@article{heitz2023iterative,
title={Iterative $\alpha$-(de) Blending: a Minimalist Deterministic Diffusion Model},
author={Heitz, Eric and Belcour, Laurent and Chambon, Thomas},
journal={arXiv preprint arXiv:2305.03486},
year={2023}
}
@article{li2023towards,
archivePrefix = {arXiv},
arxivId = {2306.09251v1},
author = {Li, Gen and Wei, Yuting and Chen, Yuxin and Chi, Yuejie},
eprint = {2306.09251v1},
journal = {arXiv preprint arXiv:2306.09251},
title = {{Towards Faster Non-Asymptotic Convergence for Diffusion-Based Generative Models}},
year = {2023}
}
